Structured Modeling of Joint Deep Feature and Prediction Refinement for Salient Object Detection

Recent saliency models extensively explore to incorporate multi-scale contextual information from Convolutional Neural Networks (CNNs). Besides direct fusion strategies, many approaches introduce message-passing to enhance CNN features or predictions. However, the messages are mainly transmitted in two ways, by feature-to-feature passing, and by prediction-to-prediction passing. In this paper, we add message-passing between features and predictions and propose a deep unified CRF saliency model . We design a novel cascade CRFs architecture with CNN to jointly refine deep features and predictions at each scale and progressively compute a final refined saliency map. We formulate the CRF graphical model that involves message-passing of feature-feature, feature-prediction, and prediction-prediction, from the coarse scale to the finer scale, to update the features and the corresponding predictions. Also, we formulate the mean-field updates for joint end-to-end model training with CNN through back propagation. The proposed deep unified CRF saliency model is evaluated over six datasets and shows highly competitive performance among the state of the arts.

==> DeletedContents.tex <==
\section{Introduction}
Visual saliency, born from psychology~\cite{koch1987shifts}, refers to the attentional selection process on the scenes by the human visual system (HVS). At its early stage, saliency detection models focused on highlighting the most conspicuous regions or eye fixations on a scene~\cite{itti1998model,harel2007graph,judd2009learning,achanta2009frequency}. Later, the connotation of \emph{saliency} was extended to the object-level prediction by emphasizing the most outstanding object on an image. Then, many salient object detection models were proposed~\cite{wei2012geodesic,yang2013saliency,mairon2014closer,jiang2015generic,liu2017hierarchical,wang2015deep,liu2016dhsnet,hou2017saliency,li2016visual}, which facilitate a broad range of computer vision applications, such as segmentation~\cite{rahtu2010segmenting}, video compression~\cite{guo2010novel}, image cropping~\cite{santella2006gaze}, video summarizing~\cite{ma2002user}, and image fusion~\cite{han2013fast}.

%\begin{figure}
%\centering
%\scalebox{0.5}{\includegraphics[width=6.6in]{./img/gestalt_example.pdf}}
%\caption{Visual comparison of side output maps from CNNs (\ie, $\textbf{f}^2$ in Section~\ref{subsec:HED}) and saliency maps from the proposed DG model. The front-end CNN rapidly locates and sketch out the salient objects (2nd row), and the cascade Gestalt CRFs apply cognitive grouping laws to refine the wrong predictions of background and the flaws from salient objects (3rd row).} 
%\label{fig:gestalt_example}
%\end{figure}

As the emergence of the convolutional neural networks (CNNs), salient object detection models receive remarkable progress in performance. 
%Early deep saliency models benefit from adjusting the inputs to deep networks such as VGG~\cite{simonyan2014very}, of which the inputs are either multi-scale re-sized images~\cite{liu2015predicting} or global and local image segments~\cite{li2016visual,wang2015deep,zhao2015saliency,kim2016shape}. 
Recent saliency models extensively explore diverse end-to-end network architectures to integrate multi-scale CNN features, \ie, the \emph{skip} structures to integrate multi-scale features~\cite{hou2017saliency}, the \emph{hierarchical} architectures to refine features from coarse scale to finer scale~\cite{liu2016dhsnet,wang2016saliency,zhang2018progressive,liu2018picanet}, and the \emph{cascade} architectures to integrate features scale by scale~\cite{zhang2017amulet}, \etc{ } 

On top of the CNN predictions, recent state of the arts~\cite{li2016deep,hou2017saliency,li2017instance} tend to add a fully connected Dense-CRF~\cite{krahenbuhl2011efficient} as a post-processing method. The Dense-CRF incorporates label agreement assumptions (\eg, similarity and proximity) as pairwise potentials into probabilistic functions of graphical models. Through the mean-field approximations, the coarse pixel-wise saliency predictions are updated based on the label agreement assumptions for fine-grained saliency maps with enhanced smoothness and sharp boundary divisions.

Different from previous saliency models using CRF for prediction refinement, we extend the CRF inference with richer pairwise potentials on both feature and prediction levels. The motivation comes from two aspects: 1) enhanced features produce better corresponding predictions; 2) more pairwise potentials provide more contextual constraints to reinforce the prediction results. Consequently, both the features and predictions can be cooperatively updated in one CRF inference for a finer saliency map.

The barriers from the existing fully connected CRFs are two folds. 1) Current Dense-CRF is disconnected from the training of CNNs such that the inference is unaware of the internal CNN features. Such disconnection blocks the potential of the front-end CNN to further optimize its features for better predictions. Thus, we formulate a novel CRF inference that facilities joint model training of the whole networks through back propagation. 2) Although Zheng~\etal~\cite{zheng2015conditional} formulate the CRF inference for joint model training on prediction level for semantic segmentation, the inference is in the discrete domain. As the CNN features must be optimized in the continuous domain, we formulate a new continuous CRF inference.

\begin{figure}
\begin{center}
\begin{minipage}{0.3\linewidth}
     \centerline{\includegraphics[width=1in]{./img/passing_1.pdf}}
     \vspace{-5pt}
     \centerline{(1)}
\end{minipage}
\begin{minipage}{0.3\linewidth}
     \centerline{\includegraphics[width=1in]{./img/passing_2.pdf}}
     \vspace{-5pt}
     \centerline{(2)}
\end{minipage}
\begin{minipage}{0.3\linewidth}
    \centerline{\includegraphics[width=1in]{./img/passing_3.pdf}}
    \vspace{-5pt}
    \centerline{(3)}
\end{minipage}
\vspace{6pt}
\caption{Cascade multi-scale refinement on 1) prediction level, 2) feature level, and 3) feature and prediction level. $\text{f}^l$ refers to the features and $\text{s}^l$ is the corresponding prediction. The arrow lines show the corresponding message passing process.}
\label{fig:passing}
\end{center}
\end{figure}

Therefore, in this paper, we design a novel 3C-CRFs saliency model, which is based on a front-end CNN with the \emph{cascade} \emph{continuous} CRFs architecture to \emph{cooperatively} integrate and refine CNN features and predictions from multiple scales for a fine-grained saliency map. In particular, at each scale, a continuous CRF block is embedded to cooperatively refine the side features as well as the side output prediction map with the contexts from the previous scale. More specifically, within a CRF inference, the current side features are updated involving their pairwise potentials with the side features and with the prediction at the previous scale, while the current prediction map is refined depending on the prediction at the previous scale, as shown in Figure~\ref{fig:passing}-(3). Then, the output refined features and the prediction map are incorporated to the continuous CRF block at the next scale. Thus, a series of continuous CRFs are constructed in a cascade flow and progressively learn a unified and refined saliency map. Moreover, the CRF inference is formulated with mean-field updates that allows jointly end-to-end training through back-propagation and no post-processing is needed. The framework of the 3C-CRFs model is presented in Figure~\ref{fig:frame}. 

In summary, a front-end CNN rapidly locates the salient objects, and the cascade continuous CRFs architecture progressively refines the side output features and predictions from coarse to finer scales for the final fine-grained saliency map. The contributions of this paper are two folds:
\begin{itemize}
\itemsep0em 
\vspace{-5pt}
  \item We propose a cascade continuous CRFs architecture that is seamlessly incorporated with the front-end CNN to progressively integrate and refine multi-scale contexts from CNNs for saliency prediction.
  \item We have made the first attempt to reformulate the CRF as cooperative feature and prediction refinement function and develop the corresponding mean-field approximation inference that supports end-to-end model training through back propagation.
  \item (might be removed)At each scale, the contributions of the pairwise potentials within the CRF can be different. Through emphasizing different pairwise potentials at different scales, the network is more flexible and can make the uttermost of the label agreement assumptions for an optimal result.
\vspace{-3pt}
\end{itemize}

With the emergence of the convolutional neural networks (CNNs), salient object detection models receive remarkable progress in performance. However, previous saliency methods model the multi-scale fusion of features and predictions separately. That is, predictions are fused with predictions~\cite{li2017instance,yu2018recurrent} (Figure~\ref{fig:passing}-1)  while features pass messages\XPC{the term message is unclear here.} to features~\cite{luo2017non,liu2018picanet,wang2018detect,chen2018progressively} (Figure~\ref{fig:passing}-2). \XPC{I would suggest moving the following sentence to Related Work.} Even both features and predictions are involved in multi-scale integration, the networks pass information separately~\cite{hou2017saliency,zhang2018bi}. In addition to separate message passing, we propose to add message passing between features and predictions to build a joint feature and prediction refinement model as Figure~\ref{fig:passing}-3. The motivations are two folds.



%The enhanced HED architecture combines both deeper and shallower side outputs from the FCNs with short connections to obtain multi-scale contexts of richer semantic features, and thus are able to better locate and sketch out the salient objects. 
%Firstly, pixels with similar appearance features are more likely to have the same labels. Secondly, neighboring pixels should possess similar labels. 
%Based on the Gestalt laws of \textit{similarity} and \textit{proximity} as post-processing approaches, previous traditional methods~\cite{wang2008two,wu2013gestalt} correct the labeling errors on the coarse saliency map by appearance and spatial coherence. For deep saliency models, the integrity of the similarity and proximity laws is also crucial in improving the quality of output maps from the FCNs. This paper aims at revisiting the classic Gestalt laws that facilitate salient object detection and reload them into deep models for refined saliency maps. 
%such as  \textit{similarity},  \textit{symmetry},  \textit{anomaly}, \textit{closure}, and \textit{Figure} \& \textit{Ground}.     


%To understand how CNNs embodies Gestalt laws, Figure~\ref{fig:gestalt_example} presents the saliency maps computed from the fully convolutional neural networks (FCNs). Apparently, the FCNs are eligible in detecting the salient objects when the organization of the visual elements on the scenes accords with the Gestalt theories such as  \textit{similarity},  \textit{symmetry},  \textit{anomaly}, and \textit{closure}. Thus, most of the Gestalt laws based on visual perception are also applicable to understand the rationale behind the CNNs.

%As a consequence, few recent works explore the assumptions or theories about photographic composition in terms of saliency because of the prevalence of the convolutional neural networks (CNNs), which however used to be the core stage in traditional saliency methods. Therefore, it is necessary to revisit the previous valuable theories about saliency from traditional methods and seek their corresponding interpretations in deep neural networks. 
%Due to the emergence of deep learning, the performance of saliency detection has been largely improved~\cite{liu2017hierarchical,wang2015deep,li2016deep,dai2016r,liu2016dhsnet,hou2017saliency,li2016visual,tang2016saliency,mahendran2016salient,lee2016deep}. These recently proposed deep saliency models break the limits of extracting handcraft features from traditional methods, such as color, intensity, orientation, textures and so forth. Instead, convolutional neural networks (CNNs) are employed to extract high-level features of rich semantics. Further, the integration of fully convolutional neural networks (FCNs) facilitates salient object detection tasks to an end-to-end phase~\cite{liu2016dhsnet,wang2016saliency,kuen2016recurrent,shengfeng2017delving,zhang2017amulet}. Recent deep saliency models, although adopts deep neural network architectures, still follow some similar saliency detection hypothesis and strategies. 
%It is notable that the convolutional neural networks are also inspired by biological processes, in which the connectivity between neurons perceives the organization of the visual cortex.  

%Firstly, the integration of multi-scale contexts is still one of the core strategies in saliency detection. Early deep saliency models construct multi-scale inputs to train the FCNs for saliency prediction, of which the inputs with multiple contexts are either the multi-scale re-sized images~\cite{liu2015predicting} or global and local contextual image segments~\cite{li2016visual,wang2015deep,zhao2015saliency,kim2016shape}. Later, as the end-to-end modeling gains much popularity, a number of deep saliency models take the advantages of the multi-scale side outputs~\cite{bruce2016deeper,zhang2017amulet,liu2016dhsnet,kuen2016recurrent} from FCNs, and adopt variable fusion strategies to produce the saliency maps.

%Secondly, the integrity of smoothing or refinement is still crucial to enhance the quality of the outputs from deep neural networks. One common approach is to integrate smoothing functions~\cite{hu2017deep,luo2017non} directly to the output layer of the FCNs. Many previous works adopt the Conditional Random Fields (CRFs) module fully connected to the FCNs to reconcile the spatial and appearance coherence on the output saliency map~\cite{li2016visual,li2017instance,hou2017saliency}. Besides, some saliency models~\cite{liu2016dhsnet,kuen2016recurrent} also embed smoothing functions to multi-scale side outputs of the FCNs as recurrent layers, such that the intermediate output maps at each scale can be refined as the inputs to the next levels of convolutional layers of the FCNs. However, previous strategies usually deploy smoothing methods to correct the labeling errors of the output map by spatial and appearance coherence at the current scale, without any considerations of the contextual information from the neighboring scales. As multi-scale contextual relationship is also informative to both refinement and multi-scale integration, a smoothing method based on multi-scale contexts is desired.    

\begin{figure*}[thbp!]
\begin{center}
\scalebox{1}{\includegraphics[width=6.8in]{./img/frame.pdf}}
\vspace{-5pt}
\caption{Framework of the 3C-CRFs saliency model. Multiple scales of side features ($\text{f}^1$$\cdots$$\text{f}^5$) and the corresponding side output prediction maps ($\text{s}^1$$\cdots$$\text{s}^5$) are extracted from the CNN. ``$\text{h}^1$$\cdots$$\text{h}^5$'' represent the estimated features and ``$\text{o}^1$$\cdots$$\text{o}^5$'' are the estimated predictions by the cascade continuous CRFs architecture. The circled symbols indicates the message passing operations within each CRF inference. 1). Message passing to estimate``$\text{h}^l$'' by convolutions: ``C'' indicates a convolutional layer followed by the corresponding deconvolutional layer, crop layer and a scale layer. 2). Message passing to estimate ``$\text{o}^l$'' with Gaussian pairwise kernels: ``G'' means the Gaussian filtering using the Permutohedral lattice implementation~\cite{adams2010fast}. ``+'' refers to element-wise sum.} 
\vspace{-5pt}
\label{fig:frame}
\end{center}
\end{figure*}

The rest of the paper is organized as follows. Section~\ref{sec:relatework} summarizes the related works. Section~\ref{sec:model} introduces the framework of the proposed 3C-CRFs saliency model. Section~\ref{sec:implementation} details the implementation. Section~\ref{sec:experiment} presents the experimental results and Section~\ref{sec:conclusion} concludes the work. 


==> comments_macro.tex <==

%dear co-authors, you may set the color assigned for you to any color you like.

%for Xiaopeng Hong
\newcommand\XP[1]{\textcolor{red}{#1}}
\newcommand\XPC[1]{\textcolor{red}{[Xiaopeng: #1]}}
\newcommand\XPDel[1]{\textcolor{red}{\sout{#1}}}
\newcommand\XPH[1]{\colorbox{red}{[#1]}}

%for Yingyue Xu
\newcommand\XYY[1]{\textcolor{blue}{#1}}

%for Wanli Ouyang
\newcommand\Ouyang[1]{\textcolor{brown}{#1}}

%for Dan Xu
\newcommand\Dan[1]{\textcolor[rgb]{0,0.5,0}{#1}}

%for Min Xu
\newcommand\Min[1]{\textcolor{purple}{#1}}

%for Guoying Zhao
\newcommand\Zhao[1]{\textcolor{orange}{#1}}

%updating
\newcommand\up[1]{\textcolor{gray}{#1}}

\def\eg{\emph{e.g.}} \def\Eg{\emph{E.g.}}
\def\ie{\emph{i.e.}} \def\Ie{\emph{I.e.}}
\def\cf{\emph{c.f.}} \def\Cf{\emph{C.f.}}
\def\etc{\emph{etc.}} \def\vs{\emph{vs.}}
\def\wrt{w.r.t.} \def\dof{d.o.f.}
\def\etal{\emph{et al.}}




==> tab/f_m_backup.tex <==
\begin{table*}[thbp!]
\begin{center}
    \begin{tabular}{c|c|ccccccccccc|c}
    \toprule
    \small{Dataset}	& \small{Metric}	& \small{DRFI}	& \small{MDF}	& \small{RFCN}	& \small{DHS}	& \small{Amulet}	& \small{UCF}	& \small{DCL$^+$}	& \small{MSR$^+$}	& \small{DSS}	& \small{DSS$^+$}	& \small{RA}	& \small{Ours}\\\midrule
    \small{MSRA-B}	&\small{maxF}	&0.851	&0.885	&-	&-	&-	&-	&0.916	&0.915	&0.920	&{0.929}	&\underline{0.931}	&\textbf{0.935}\\
    	&\small{MAE}	&.123	&.066	&-	&-	&-	&-	&.047	&.053	&.043	&\underline{.034}	&.036	&\textbf{.029}\\\midrule
    \small{PASCAL-S}	&\small{maxF}	&.690	&.764	&.832	&.824	&.832	&.818	&.822	&.833	&.826	&\underline{.835}	&.834	&\textbf{.864}\\
    	&\small{MAE}	&.210	&.145	&.118	&\underline{.094}	&.100	&.116	&.108	&\underline{.094}	&.102	&.095	&.104	&\textbf{.087}\\\midrule
    \small{DUT-}	&\small{maxF}	&.664	&.694	&.747	&-	&.743	&.730	&.757	&.777	&.764	&.781	&\underline{.786}	&\textbf{.802}\\
    \small{OMRON}	&\small{MAE}	&.150	&.092	&.095	&-	&.098	&.120	&.080	&.078	&.072	&.063	&\underline{.062}	&\textbf{.056}\\\midrule
    \small{HKU-IS}	&\small{maxF}	&.775	&.861	&.896	&.892	&.899	&.888	&.904	&\underline{.916}	&.900	&\underline{.916}	&.913	&\textbf{.924}\\
    	&\small{MAE}	&.146	&.076	&.073	&.052	&.050	&.061	&.049	&\underline{.040}	&.050	&\underline{.040}	&.045	&\textbf{.035}\\\midrule
    \small{ECSSD}	&\small{maxF}	&.784	&.847	&.899	&.907	&.914	&.902	&.901	&.907	&.908	&\underline{.919}	&.918	&\textbf{.928}\\
    	&\small{MAE}	&.172	&.106	&.091	&.059	&.061	&.071	&.068	&.062	&.062	&\underline{.055}	&.059	&\textbf{.050}\\\midrule
    \small{ICoseg}	&\small{maxF}	&.812	&.838	&.846	&.851	&\textbf{.899}	&.884	&.875	&.852	&.860	&.872	&.868	&\underline{.895}\\
    	&\small{MAE}	&.145	&.101	&.097	&.070	&.070	&.068	&\underline{.066}	&.071	&.075	&.068	&.082	&\textbf{.062}\\
    \bottomrule
    \end{tabular}
    \vspace{5pt}
    \caption{Evaluation results on six dataset and with models DRFI~\cite{jiang2013salient}, MDF~\cite{li2015visual}, RFCN~\cite{wang2016saliency}, DHS~\cite{liu2016dhsnet}, Amulet~\cite{zhang2017amulet}, UCF~\cite{zhang2017learning}, DCL~\cite{li2016deep}, MSR~\cite{li2017instance}, DSS~\cite{hou2017saliency}, RA~\cite{chen2018reverse} and the proposed deep CRF model. ``$+$'' marks the models utilizing Dense-CRF~\cite{krahenbuhl2011efficient} for post-processing. ``-'' means that the corresponding dataset is used as the training data. The evaluation on MSRA-B is performed on the testing set.}
    \vspace{-15pt}
    \label{tbl:f_m}
\end{center}
\end{table*} 

==> tab/layer.tex <==
\begin{table*}
\small
\begin{center}
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
    \hline
    \footnotesize{Level}&\footnotesize{Layer}&\footnotesize{Size}&\footnotesize{conv\_1}&\footnotesize{conv\_2}&\footnotesize{conv\_3}&\footnotesize{Size}&\footnotesize{Concatenate}&\footnotesize{Size}&\footnotesize{Contexts}&\footnotesize{CRF} \\\hline
    %1&  conv1\_2&    64,248$\times$328&    128,3$\times$3&   128,3$\times$3&   1,1$\times$1&    1,248$\times$328& 1,3,4,5&   1,240$\times$320&    $C_5$& $R_5$  \\
    1&  conv2\_2&    128,124$\times$164&    128,3$\times$3&   128,3$\times$3&   1,1$\times$1&    1,124$\times$164& 2,3,4,5&   1,240$\times$320&    $c^5$&    $R_5$\\
    2&  conv3\_3&    256,62$\times$82&    256,5$\times$5&   128,5$\times$5&   1,1$\times$1&    1,62$\times$82& 3,4,5&   1,240$\times$320&    $c^4$&    $R_4$\\
    3&  conv4\_3&    512,31$\times$41&    256,5$\times$5&   128,5$\times$5&   1,1$\times$1&    1,31$\times$41& 4,5&   1,240$\times$320&    $c^3$&    $R_3$\\
    4&  conv5\_3&    512,16$\times$21&    512,5$\times$5&   128,5$\times$5&   1,1$\times$1&    1,16$\times$21&-&   1,240$\times$320&     $c^2$&    $R_2$\\
    5&  pool5&    512,9$\times$11&    512,7$\times$7&   128,7$\times$7&   1,1$\times$1&    1,9$\times$11&-&   1,240$\times$320&     $c^1$&    -\\
    \hline
    \end{tabular}
    \caption{Detailed implementation of short connections to side outputs of VGGNet. The parameters for convolutional layers are formulated as (channel, kernel size) and the output sizes (``Size'') are expressed as (channel, output size).}
    \label{tbl:layer}
\end{center}
\end{table*} 

==> tab/param_full.tex <==
\begin{table}
\small
\begin{center}
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \hline
    $T$	&$\sigma_\alpha$&$\sigma_\beta$	&$\sigma_\gamma$	&$\nu_1$	&$\nu_2$	&F-mesure&MAE\\\hline\hline
    6	&1	&1	&1	&1	&1	&0.8918	&0.0706\\
    3	&1	&1	&1	&1	&1	&0.8918	&0.0710\\
    20	&1	&1	&1	&1	&1	&0.8915	&0.0707\\
    6	&10	&10	&10	&1	&1	&\underline{0.9090}	&0.0707\\
    6	&10	&1	&1	&1	&1	&0.8963	&0.0843\\
    6	&1	&10	&1	&1	&1	&0.8933	&\underline{0.0701}\\
    6	&1	&1	&10	&1	&1	&0.8920	&0.0703\\
    6	&10	&10	&1	&1	&1	&\textbf{0.9092}	&0.0943\\
    6	&1	&10	&10	&1	&1	&0.8935	&\textbf{0.0698}\\
    6	&10	&1	&10	&1	&1	&0.8958	&0.0948\\
    6	&1	&1	&1	&3	&5	&0.8918	&0.0706\\
    6	&1	&1	&1	&5	&3	&0.8918	&0.0706\\
    6	&30	&15	&3	&3	&5	&0.9059	&0.0749\\\hline\hline
    3	&20	&20	&1	&1	&1	&0.9061	&0.0876\\
    6	&20	&20	&1	&1	&1	&0.9069	&0.0797\\
    6	&20	&20	&1	&3	&5	&0.9069	&0.0797\\
    6	&20	&10	&1	&1	&1	&0.9087	&0.0808\\
    6	&20	&10	&1	&3	&5	&0.9087	&0.0808\\
    6	&10	&5	&1	&1	&1	&0.9084	&0.0961\\
    6	&10	&5	&1	&3	&5	&0.9084	&0.0961\\
    6	&1	&1	&10	&1	&1	&0.8920	&0.0703\\
    6	&1	&1	&10	&3	&5	&0.8920	&0.0703\\
    6	&1	&1	&20	&1	&1	&0.8920	&0.0707\\
    6	&1	&1	&20	&3	&5	&0.8920	&0.0707\\
    3	&1	&1	&10	&1	&1	&0.8921	&0.0703\\
    4	&1	&1	&10	&1	&1	&0.8921	&0.0703\\
    5	&1	&1	&10	&1	&1	&0.8920	&0.0703\\
    6	&5	&5	&1	&1	&1	&0.9027	&0.0942\\
    6	&5	&1	&1	&1	&1	&0.8935	&0.0745\\
    6	&1	&1	&5	&1	&1	&0.8924	&0.0700\\
    \hline
    \end{tabular}
    \caption{$T$ refers to the number of iterations by mean-field iterations. The appearance kernel is controlled by $\sigma_\alpha$ and $\sigma_\beta$ and the weight $\nu_1$, while the smoothness kernel is controlled by $\sigma_\gamma$ and the weight $\nu_2$. $\tau$ refers to the scale parameter for normalization. \XP{which dataset we used here?}}
    \label{tbl:param}
\end{center}
\end{table} 

==> tab/pseudocode.tex <==
\begin{algorithm}
  \caption{Mean-field Approximation}
  \label{pseudo}
  \begin{algorithmic}
  \State ${\rho}_{l,m}=\sum_{j\neq i}K_m^{ij}$ \Comment{Normalization Matrix}
  \While{not converged} 
  \State $\tilde{\mu}_{l,m}^{t}=\sum_{j\neq i}(K_m^{ij}\mu_{l,m}^{t}-\mu_{l,m}^{t})$ \\ \Comment{Message Passing}
  %\NoNumber{$\tilde{\mu}_{l,m}^{t}=\sum_{j\neq i}K_m^{ij}\mu_{l,m}^{t}$} 
  \State ${\rho_l}=2\sum_m(\beta_m {\rho}_{m}-1)$   
  \State $\breve{\mu}_{l}^{t}=2\sum_{m}\beta_m \tilde{\mu}_{l,m}^{t}$
  \\ \Comment{Weighting Filter Output}
  \State $\bar{\mu}_{l}^{t}=c_l+\breve{\mu}_{l}^{t}$
  \\ \Comment{Adding Unary Term}
  \State ${\mu}_{l}^{t}=\bar{\mu}_{l}^{t}/{\rho_l}$
  \\ \Comment{Normalization}
  \EndWhile
%  \State $p \in [0,1]$, $G$
%  \State None \Comment{a test comment}
%  \For{$i = 0 \to 2^d-1$}\Comment{another test comment} 
%    \If{$n(\nu_i) = 0$}
%      \If{ $x < p$}  \Comment{$x$ is a normal distribution number in the range of $[0,1]$}
%      \State Occupy $v_i$ site with probablility $p$ 
 %     \EndIf
 %   \EndIf
 % \EndFor
  \end{algorithmic}
\end{algorithm}
